Systematic Unsupervised Recycled Field-Programmable Gate Array Detection

With the expansion of the semiconductor supply chain, the use of recycled field-programmable gate arrays (FPGAs) has become a serious concern. Several methods for detecting recycled FPGAs by analyzing the ring oscillator (RO) frequencies have been proposed; however, most assume the known fresh FPGAs (KFFs) as the training data in machine-learning-based classification. In this study, we propose a novel recycled FPGA detection method based on an unsupervised anomaly detection scheme when there are few or no KFFs available. As the RO frequencies in the neighboring logic blocks on an FPGA are similar because of systematic process variation, our method compares the RO frequencies and does not require KFFs. The proposed method efficiently identifies recycled FPGAs through outlier detection using direct density ratio estimation. Experiments using Xilinx Artix-7 FPGAs demonstrate that the proposed method successfully distinguishes recycled FPGAs from 35 fresh FPGAs. In contrast, a conventional recycled FPGA detection method results in certain misclassification.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/i2.eps}}]{Yuya Isaka}
received B.E. degree from Kwansei Gakuin University, Japan, in 2021.
Currently, he is pursuing a master's degree at the Graduate School of
Information Science, Nara Institute of Science and Technology (NAIST),
Japan. His research interests include counterfeit field programmable gate
array (FPGA) detection, hardware security and reliability, very large-scale
integration (VLSI) testing, and dependability-aware RISC-V design.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/s1.eps}}]{Michihiro Shintani}
received B.E. and M.E. degrees from Hiroshima City University,
Hiroshima, Japan, and a Ph.D. degree from Kyoto University, Kyoto,
Japan, in 2003, 2005, and 2014, respectively. He was with Panasonic
Corporation, Osaka, Japan, from 2005 to 2014; with Semiconductor
Technology Academic Research Center (STARC), Yokohama, Japan, from
2008 to 2010; with Kyoto University, Kyoto, Japan, from 2014 to 2017;
and with Nara Institute of Science and Technology (NAIST), Ikoma,
Japan, from 2017 to 2022. In 2022, he joined the Department of
Electronics, Kyoto Institute of Technology, Kyoto, Japan, where he is
currently an Associated Professor.  His research interests include
reliability-aware circuit design, device modeling, and circuit
simulation for VLSI and power converters.  He is a senior member of
IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/f1.eps}}]{Foisal Ahmed}
has completed his Ph.D. degree at the Graduate School of Information
Science, Nara Institute of Science and Technology (NAIST), Japan, in
2020. Previously, he received B.E. degree from Prime University,
Dhaka, in 2008; P.G.D. degree from Bangladesh University of
Engineering and Technology (BUET), Dhaka, in 2014 and M.E. degree from
Islamic University of Technology (IUT), Dhaka, Bangladesh, in
2016. Currently, he is working as a postdoc researcher in the Computer
Systems Department, Tallinn University of Technology, Tallinn,
Estonia. His research interests include hardware security,
reliability, very large-scale integration (VLSI) testing, signal
processing, and communications systems. He is a member of IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/m1.eps}}]{Michiko Inoue}
received her B.E., M.E., and Ph.D. degrees in Computer Science from
Osaka University, Japan in 1987, 1989, and 1995 respectively.  She
worked at Fujitsu Laboratories Ltd. from 1989 to 1991. She is a
Professor of Graduate School of Science and Technology, Nara institute
of Science and Technology (NAIST). Her research interests include
distributed algorithms, graph theory and dependability of digital
systems. She is a member of Science Council of Japan, the Information
Process- ing Society of Japan (IPSJ), and Japanese Society for
Artificial Intelligence, a senior member of IEEE, and a fellow of the
Institute of Electronics, Information and Communication Engineers
(IEICE).
\end{IEEEbiography}

